Evaluating Manual Intervention to Address the Challenges of Bug Finding with KLEE

Symbolic execution has shown its ability to find security-relevant flaws in software, but faces significant scalability challenges. There is a commonly held belief that manual intervention by an expert can help alleviate these limiting factors. However, there has been little formal investigation of this idea. In this paper, we present our experiences applying the KLEE symbolic execution engine to a new bug corpus, and of using manual intervention to alleviate the issues encountered. Our contributions are (1) Hemiptera, a novel corpus of over 130 bugs in real world software, (2) a comprehensive evaluation of the KLEE symbolic execution engine on Hemiptera with a categorisation of frequently occurring software patterns that are problematic for symbolic execution, and (3) an evaluation of manual mitigations aimed at addressing the underlying issues of symbolic execution. Our experience shows that manual intervention can increase both code coverage and bug detection in many situations. It is not a silver bullet however, and we discuss its limitations and the challenges encountered.

==> sections/challenges/2_semantically_equivalent.tex <==
% John

%2) Loop + condition constructs searching for a constant where the produced states are “semantically equivalent”
%	-> Environment.
%	-> Application.

During our analysis, we also came across code constructs which result in forking semantically similar states. A multitude of such states provides no benefit with future exploration, and consequently should be removed so that computation can be prioritised elsewhere. 

\begin{lstlisting}[label={code:imginfocode1},caption={Excessive State forking due to skipping of comments.}]
do {
  switch (c = jas_stream_getc(in)) {
    ...
    case '#':
      for (;;) {
        if ((c = jas_stream_getc(in)) == EOF) {
          done = 1;
          break;
        }
        if (c == '\n') { break; }
      }
      break;
   	  ...
    }
} while (!done);
\end{lstlisting}

One code construct associated with this issue is often found in parsing functions. Essentially, it involves reading data from a symbolic source, via a loop, in search for a particular constant, while ignoring anything else. Listing \ref{code:imginfocode1} provides an example of such a case. The code is taken from the function, \ic{mif\_getc}, and is part of ImgInfo (a binary included the JasPer project). It includes a loop to skip over any comments, which start with '\#' and end with a new-line or end-of-file character. Given the terminating condition in the while loop, namely \ic{ch != '{\textbackslash}n' \&\& ch != EOF}, numerous semantically similar states, which only differ in the length of the ignored comment, are forked. According to our results, the code causes 73.97\% of all forks. The solution to this problem is to insert an assumption that implies comments are not present, i.e.\ \ic{klee\_assume(c != '\#')}.  Assumptions affect completeness, but not correctness, so are safe to add at the cost of unexplored regions.

Libjpeg-turbo has a similar code construct used to skip any trailing white characters present before numbers in a file. Again, we addressed this issue by inserting an assumption, as shown in listing \ref{code:libjpegcode2}.

\begin{lstlisting}[label={code:libjpegcode2},caption={Excessive State forking due to skipping of trailing white characters (includes added assumption).}]
/* Skip any leading whitespace */
do {
  ch = pbm_getc(infile);

  klee_assume(ch >= '0' & ch <= '9');
...
} while (ch == ' ' || ch == '\t' || ch == '\n' || ch == '\r');
\end{lstlisting}

==> sections/challenges/3_unbounded_loop_bounds.tex <==
% John
% Unbounded symbolic data being used as loops bounds

Loops unbounded due to symbolic data are problematic, especially if the states produced are not semantically similar and are of interest in terms of future exploration.One viable solution is to constrain a loop to an upper-bound, in order to circumvent the state-explosion problem, at the expense of completeness. Listing \ref{code:libjpeg-code3} illustrates a code fragment taken from libgjpeg, and is a case example that highlights the challenge. The code initializes the variable \ic{maxval} with an integer read from file. As seen at line 19, \ic{maxval} is then used as an upper-bound  for a loop. This results in producing a large number of states that amounts to 14.83\% of all forking on an experimental run. We undertake this challenge by assuming four possible values for \ic{maxval}, namely \ic{MAXJSAMPLE}, 100, 255 and 300. The reason behind the selection of these values
stems from condition statements present further up in the function, such as at line 10.

\begin{lstlisting}[label={code:libjpeg-code3},caption={Excessive state forking due to Unbounded Loop}]
...:
maxval = read_pbm_integer(cinfo, source->pub.input_file);

klee_assume(maxval == MAXJSAMPLE | maxval == 100 | maxval == 255 | maxval == 300 );

switch (c) {
  ...
  case '5':
    ...
    if (maxval > 255) {
      ...
    } else if (maxval == MAXJSAMPLE && SIZEOF(JSAMPLE) == SIZEOF(U_CHAR)) {
      ...
    } else {
      ...
    }
  }
...
 for (val = 0; val <= (INT32) maxval; val++) {
      source->rescale[val] = (JSAMPLE) ((val*MAXJSAMPLE + half_maxval)/maxval);
    }
  }
...
\end{lstlisting}



==> sections/challenges/5_inordinately_expensive.tex <==
% Dan

%5) Inordinately expensively, but potentially relevant code (zlib: bits < 15)
%	-> Case split / Trade off / Time vs reward (tcpdump, libtiff, imginfo, etc.)
%
% Emphasis on case split.

%Programs often contain code blocks that are very expensive to analyse symbolically, such is the nature of symbolic execution.  This is a core problem of the technique.

%Many programs under analysis have very large analysis complexity in at least some code blocks.  In Section \ref{sec:challenges_semantic_independence} which considered the case of code  which was semantically independent from later code, these code blocks instead have a direct correspondence to later code and to remove them ehttps://www.overleaf.com/7965371zxcghgzkjrbs#ntirely would affect effectiveness.

In Section \ref{sec:challenges_semantic_independence} we considered the case of code  which was semantically independent from later code, and hence could be reduced or removed.  However, many programs under analysis have code blocks with very large analysis complexity that are \emph{not} semantically independent from future blocks.  This cannot be removed entirely whilst maintaining complete semantics.


Nevertheless, some of these  blocks contain a branch which splits program analysis into two similar but distinct problems.  It is not unusual that one is so expensive that to analyse both cases simultaneously would likely result in a very low reward for time invested.  A specific case of this is a program which can read in two or more different formats into an internal data structure, and then modifies this data structure directly.  Each case is likely to lead to different challenges later in the program, so splitting this into two analysis cases could be far more effective.  This paradigm is common and exists in \ic{LIBpcap}, \ic{flac} and others.


\begin{lstlisting}[label={code:fread_in_pcap_1},caption={}]
amt_read = fread((char *)&magic, 1, sizeof(magic), fp);                  
/** Try all file types. */  
for (i = 0; i < N_FILE_TYPES; i++) {                                     
	p = (*check_headers[i])(...);     
	if (p != NULL) {                                                
		goto found;                                              
} /* ... */                                                                 
\end{lstlisting}

The \ic{check\_headers} call in Listing \ref{code:fread_in_pcap_1} eventually calls the code in Listing \ref{code:check_headers_in_pcap_2}.

\begin{lstlisting}[label={code:check_headers_in_pcap_2},caption={}]
if (magic != TCPDUMP_MAGIC 
	&& magic != KUZNETZOV_TCPDUMP_MAGIC 
	&& magic != NSEC_TCPDUMP_MAGIC) {                                       
	magic = SWAPLONG(magic);                                         
	if (magic != TCPDUMP_MAGIC && 
    	magic != KUZNETZOV_TCPDUMP_MAGIC 
        && magic != NSEC_TCPDUMP_MAGIC)                                 
        	return (NULL);  /* nope */                               
		swapped = 1;                                                     
}  
\end{lstlisting}

The focus for the analyst may be to drive states through this code as efficiently as possible.  This may provide more rewarding symbolic execution.  To enable this, the analyst should constraint a single filetype (and hence path) via an \ic{assume} statement.  In Listing \ref{code:fread_in_pcap_1}, the iterator generates a large number of state forks by considering all possible file types.  Each of these forks in turn has a significant amount of expensive analysis that is simply unrewarding to perform simultaneously.  Instead, the state-space can be split into multiple analysis runs, one for each input file type.

An example constraint could be: \\
\ic{klee\_assume(magic == TCPDUMP\_MAGIC)}.


There are several subjective challenges here.  Firstly it is necessary to identify code which is expensive and must be reduced, secondly it must be determined whether a natural case split occurs, and thirdly, the analyst must choose which case to maintain initially, although they can change this for further analysis.

 % needs moore bigtiff?

% Semantic DEPENDENCE.
% Complexity for one section either now or later
% reward low.
% makes sense to split the problem into two, or sim

% BigTIFF

==> sections/modification_results.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[t]
% \centering
% \caption{The coverage and bugs discovered when running \KLEE~ on our modified programs.}
% \label{tab:final_results}
% \begin{tabular}{|l|l|r|r|r|r|r|r|r|r|}
% \hline
% \multirow{3}{*}{\textbf{Binary}} & \multirow{3}{*}{\textbf{Commit}} & \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Default \\ State of the Art\end{tabular}}}} & \multicolumn{6}{c|}{\textbf{After Modifications}}                                                                    \\ \cline{5-10} 
%                                  &                                  & \multicolumn{2}{c|}{}                                                                                              & \multicolumn{3}{c|}{\textbf{Bugs}}                     & \multicolumn{3}{c|}{\textbf{ICoverage}}                     \\ \cline{3-10} 
%                                  &                                  & \textbf{Bug average}                                        & \textbf{ICov}                                        & \textbf{Mean} & \textbf{Change} & \textbf{Change (\%)} & \textbf{Mean} & \textbf{Change (pp)} & \textbf{Change (\%)} \\ \hline
% libjpeg                          & 3091354                          & 1                                                           & 15.01                                                & 1             & 0               & 0\%                  & 21.46         & +6.45pp              & +42.97\%             \\ \hline
% libjpeg                          & a0b7de9*                         & 0                                                           & 23.1                                                 & 0             & 0               & 0\%                  & 27.08         & +3.98pp              & +17.23\%             \\ \hline
% imginfo                          & b702259                          & 1                                                           & 10.39                                                & 1.67          & 0.67            & +67\%                & 11.3          & +0.91pp              & +8.76\%              \\ \hline
% imginfo                          & 4212e7e*                         & 0                                                           & 10.36                                                & 0             & 0               & 0\%                  & 14.22         & +3.86pp              & +37.26\%             \\ \hline
% file                             & df74b09*                         & 0                                                           & 12.61                                                & 0             & 0               & 0\%                  & 16.62         & +4.01pp              & +31.80\%             \\ \hline
% file                             & b6e8437                          & 0                                                           & 13.83                                                & 1             & 1               & +100\%               & 16.25         & +2.42pp              & +17.50\%             \\ \hline
% tcpdump                          & 17a3c288*                        & 32                                                          & 4.94                                                 & 61.3          & 29.3            & +92\%                & 8.89          & +3.95pp              & +79.96\%             \\ \hline
% tcpdump                          & a9e4211                          & 40                                                          & 4.91                                                 & 69.3          & 29.3            & +73\%                & 10.03         & +5.12pp              & +104.28\%            \\ \hline
% zlib                             & 7c2a874                          & 0                                                           & 26.56                                                & 1             & 1               & +100\%               & 33.83         & +7.27pp              & +27.37\%             \\ \hline
% zlib                             & cacf7f1d*                        & 0                                                           & 26.7                                                 & 0             & 0               & 0\%                  & 30.66         & +3.96pp              & +14.83\%             \\ \hline
% tiff2pdf                         & f64949a                          & 0                                                           & 8.42                                                 & 0             & 0               & 0\%                  & 9.17          & +0.75pp              & +8.91\%              \\ \hline
% tiff2pdf                         & d57ccfc9*                        & 0                                                           & 8.48                                                 & 0             & 0               & 0\%                  & 7.68          & -0.80pp              & -9.43\%              \\ \hline
% flac                             & d8d1717                          & 0                                                           & 12.29                                                & 1             & 1               & +100\%               & 17.3          & +5.01pp              & +40.76\%             \\ \hline
% flac                             & d2cb0d1*                         & 0                                                           & 12.48                                                & 0             & 0               & 0\%                  & 17.3          & +4.82pp              & +38.62\%             \\ \hline
% w3m                              & 1ac245b*                         & 0                                                           & 9.01                                                 & 0             & 0               & 0\%                  & 9.43          & +0.42pp              & +4.66\%              \\ \hline
% w3m                              & 02ba3d6                          & 4                                                           & 9.07                                                 & 5             & 1               & +25\%                & 9.13          & +0.06pp              & +0.66\%              \\ \hline
% w3m-driver                       & 1ac245b                          & NA                                                          &                                                      & 0             &                 &                      &               &                      &                      \\ \hline
% w3m-driver                       & 02ba3d6                          & NA                                                          &                                                      & 24            &                 &                      &               &                      &                      \\ \hline
% \multicolumn{5}{|l|}{\textbf{Average change}}                                                                                                                                                            & +3.95pp         & +0.35pp              &               & +3.26pp              & +29.13\%             \\ \hline
% \end{tabular}
% \end{table}

==> sections/quantitative_res.tex <==
\begin{table*}[tbp]
\centering
\caption{My caption}
\label{my-label}
\begin{tabular}{llllllll}
Program     & Commit          & \begin{tabular}[c]{@{}l@{}}Bugs \\ Found \#1\end{tabular} & \begin{tabular}[c]{@{}l@{}}Bugs \\ Found \#2\end{tabular} & \begin{tabular}[c]{@{}l@{}}Bugs \\ Found \#3\end{tabular} & \begin{tabular}[c]{@{}l@{}}Average \\ Icov\end{tabular} & \begin{tabular}[c]{@{}l@{}}Average \\ Bcov\end{tabular} & \begin{tabular}[c]{@{}l@{}}Average\\ Mem (MB)\end{tabular} \\
imginfo    & b702259         & 3                                                         & 2                                                         & 2                                                         & 9.69\%                                                  & 9.12\%                                                  & 2814                                                       \\
imginfo    & 4212e7e         & 0                                                         & 0                                                         & 0                                                         & 12.14\%                                                 & 11.55\%                                                 & 2810                                                       \\
tcpdump    & a9e4211         & 7                                                         & 0                                                         & 0                                                         & 4.63\%                                                  & 3.33\%                                                  & 4750                                                       \\
tcpdump    & 8322d3a         & 0                                                         & 0                                                         & 0                                                         & 4.03\%                                                  & 2.95\%                                                  & 3192                                                       \\
tcpdump    & 17a3c288        & 0                                                         & 0                                                         & 0                                                         & 4.03\%                                                  & 2.93\%                                                  & 2710                                                       \\
jasper     & ed355a6         & 0                                                         & 0                                                         & 0                                                         & 12.03\%                                                 & 11.34\%                                                 & 2747                                                       \\
jasper     & 4212e7e         & 0                                                         & 0                                                         & 0                                                         & 13.60\%                                                 & 12.53\%                                                 & 3206                                                       \\
djpeg      & 3091354         & 0                                                         & 0                                                         & 0                                                         & 11.43\%                                                 & 10.07\%                                                 & 2320                                                       \\
djpeg      & a0b7de9         & 0                                                         & 0                                                         & 0                                                         & 8.76\%                                                  & 9.26\%                                                  & 2490                                                       \\
minigzip   & head            & 0                                                         & 0                                                         & 0                                                         & 20.47\%                                                 & 16.52\%                                                 & 136                                                        \\
minigzip   & 14763ac         & 0                                                         & 0                                                         & 0                                                         & 24.82\%                                                 & 19.14\%                                                 & 2323                                                       \\
minigzip   & 7c2a874         & 0                                                         & 0                                                         & 0                                                         & 19.93\%                                                 & 16.10\%                                                 & todo                                                       \\
tiff2bw    & cd82b52         & 0                                                         & 0                                                         & 0                                                         & 9.27\%                                                  & 7.61\%                                                  & 6522                                                       \\
tiffcmp    & 9ec1d40         & 0                                                         & 0                                                         & 0                                                         & 8.86\%                                                  & 7.25\%                                                  & 2526                                                       \\
tiffcp     & 9ec1d40         & 0                                                         & 0                                                         & 0                                                         & 9.58\%                                                  & 8.03\%                                                  & 1144                                                       \\
tiffcp     & f64949a         & 0                                                         & 0                                                         & 0                                                         & 9.33\%                                                  & 7.78\%                                                  & 2357                                                       \\
tiffset    & cd82b52         & 0                                                         & 0                                                         & 0                                                         & 8.54\%                                                  & 7.18\%                                                  & 3392                                                       \\
rgb2ycbcr  & cd82b52         & 0                                                         & 0                                                         & 0                                                         & 8.86\%                                                  & 7.78\%                                                  & 1816                                                       \\
thumbnail  & cd82b52         & 0                                                         & 0                                                         & 0                                                         & 9.50\%                                                  & 7.76\%                                                  & 2269                                                       \\
tiff2pdf   & 18b29a6         & 0                                                         & 0                                                         & 0                                                         & 6.40\%                                                  & 6.27\%                                                  & 518                                                        \\
tiff2pdf   & 8b4c419         & 0                                                         & 0                                                         & 0                                                         & 9.19\%                                                  & 8.24\%                                                  & 423                                                        \\
tiff2pdf   & 9ec1d40         & 0                                                         & 0                                                         & 0                                                         & 7.02\%                                                  & 6.52\%                                                  & 2405                                                       \\
tiff2pdf   & cd82b52         & 0                                                         & 0                                                         & 0                                                         & 7.12\%                                                  & 6.51\%                                                  & 3529                                                       \\
tiff2pdf   & f64949a         & 0                                                         & 0                                                         & 0                                                         & 7.40\%                                                  & 6.77\%                                                  & 2646                                                       \\
tiff2rgba  & cd82b52         & 0                                                         & 0                                                         & 0                                                         & 8.50\%                                                  & 7.61\%                                                  & 1422                                                       \\
tiffcp     & f64949a         & 0                                                         & 0                                                         & 0                                                         & 9.27\%                                                  & 7.89\%                                                  & 3165                                                       \\
tiffcrop   & cd82b52         & 0                                                         & 0                                                         & 0                                                         & 7.54\%                                                  & 6.35\%                                                  & 3177                                                       \\
tiffcrop   & f64949a         & 0                                                         & 0                                                         & 0                                                         & 7.64\%                                                  & 6.17\%                                                  & 2339                                                       \\
tiffinfo   & cd82b52         & 0                                                         & 0                                                         & 0                                                         & 8.95\%                                                  & 7.54\%                                                  & 2207                                                       \\
tiffinfo   & f64949a         & 0                                                         & 0                                                         & 0                                                         & 9.13\%                                                  & 7.69\%                                                  & 3324                                                       \\
tiffsplit  & cd82b52         & 0                                                         & 0                                                         & 0                                                         & 8.62\%                                                  & 7.13\%                                                  & 3758                                                       \\
tiffsplit  & f64949a         & 0                                                         & 0                                                         & 0                                                         & 8.54\%                                                  & 7.11\%                                                  & 3376                                                       \\
tiffcrop   & f64949a         & 0                                                         & 0                                                         & 0                                                         & 7.63\%                                                  & 6.43\%                                                  & 3319                                                       \\
tiffmedian & f64949a         & 0                                                         & 0                                                         & 0                                                         & 8.79\%                                                  & 7.21\%                                                  & 3313                                                       \\
tiffinfo   & cd82b52         & 0                                                         & 0                                                         & 0                                                         & 9.13\%                                                  & 7.57\%                                                  & 2206                                                       \\
file       & 4a51454         & 0                                                         & 0                                                         & 0                                                         & 15.00\%                                                 & 9.97\%                                                  & 1709.513333                                                \\
file       & 7445748         & 0                                                         & 0                                                         & 0                                                         & 14.61666667                                             & 9.76                                                    & 2091.45                                                    \\
file       & ba9a661         & 0                                                         & 0                                                         & 0                                                         &                                                         &                                                         &                                                            \\
file       & ba9a661-marg    & 0                                                         & 0                                                         & 0                                                         &                                                         &                                                         &                                                            \\
file       & b6e8437-symarg- & 0                                                         & 0                                                         & 0                                                         & 15.68666667                                             & 10.28333333                                             & 24125                                                      \\
w3m        & 06caca1         & 2                                                         & 2                                                         & 2                                                         & 8.15                                                    & 6.01                                                    & 1417.35                                                   
\end{tabular}
\end{table*}

==> sections/sota_comparisons.tex <==
\begin{table}[tbp]
\centering
\caption{My caption TODO}

\begin{tabular}{l|r|r|}
\cline{2-3}
 & \multicolumn{1}{l|}{\textbf{Bug Mean}} & \multicolumn{1}{l|}{\textbf{ICov}} \\ \hline
\multicolumn{1}{|l|}{\textbf{SOTA}} & 4.54 & 13.38\% \\ \hline
\multicolumn{1}{|l|}{\textbf{SOTA + Random Path}} & 0.25 & 13.66\% \\ \hline
\multicolumn{1}{|l|}{\textbf{SOTA + Random Fork}} & 3.58 & 13.17\% \\ \hline
\end{tabular}
\label{tab:sota}
\end{table}
